Rethinking electrified transportation: The case for dynamic wireless charging

Long-term infrastructure investment often requires choosing between an established technology and a capital-intensive alternative that gains value as demand matures. For electric vehicle (EV) charging, this trade-off is between incumbent stationary charging technology and emerging dynamic wireless charging (DWC). DWC could fundamentally alter transportation electrification by enabling high-throughput charging in motion and reducing reliance on large onboard batteries; however, its high upfront cost makes the timing and location of deployment critical. Overcommitting to stationary charging stations (SCS) risks technological lock-in and forgoing the benefits of DWC, whereas premature DWC deployment can strand capital in underutilized corridors. Through a joint investment assessment framework coupling DWC, SCS, and supporting grid infrastructure across nearly 49,000 miles of the US Interstate freight network, we find that higher utilization and longer project lifetimes rapidly shift investment toward DWC, whose share rises sharply from 48% at a project lifetime of 30 years to 100% at 32 years. Contiguous DWC segments can share grid connections, enabling them to provide over six times the rated charging capacity of SCS while requiring 46% less investment in new distribution-grid infrastructure. We also find that a combined DWC and SCS portfolio reaches a maximum lifetime value of USD 60 billion, 63% above the case with only SCS. We further identify specific traffic demand, construction, and grid access conditions that shape where each technology becomes advantageous, yielding actionable thresholds for SCS and DWC deployment that directly inform long-term EV charging infrastructure investment and policy.

==> latexmkrc <==
# Standalone documents obtain opposite-part labels from a native combined build.
# This removes the circular main/SI compilation dependency. No shell escape.
use File::Spec;
use File::Basename qw(basename);
my $root = basename($ARGV[-1] // '');
my $reference_dir = $out_dir || '.';
for my $arg (@ARGV) {
    $reference_dir = $1 if $arg =~ /^-(?:outdir|output-directory)=(.+)$/;
}
if (!$ENV{DWC_REFERENCE_BUILD} && $root =~ /^(sn-article|Supplementary_main)(\.tex)?$/) {
    local $ENV{DWC_REFERENCE_BUILD} = 1;
    my @command = ('latexmk', '-pdf', '-interaction=nonstopmode', '-halt-on-error');
    push @command, "-outdir=$reference_dir";
    push @command, 'combined.tex';
    system(@command) == 0 or die "Combined reference build failed\n";
    my $dir = $reference_dir;
    open my $source, '<', File::Spec->catfile($dir, 'combined.aux') or die $!;
    open my $main, '>', File::Spec->catfile($dir, 'crossref-main.aux') or die $!;
    open my $si, '>', File::Spec->catfile($dir, 'crossref-si.aux') or die $!;
    while (my $line = <$source>) {
        next unless $line =~ /^\\newlabel\{([^}]+)\}/;
        # Methods retain their former si- label names after relocation.
        # Classify by the actual supplementary hyperlink destination.
        my $target = $line =~ /\{[^{}]*\.supp\./ ? $si : $main;
        print {$target} $line;
    }
    close $source; close $main; close $si;
}

